Recognizing Geometric Intersection Graphs Stabbed by a Line

In this paper, we determine the computational complexity of recognizing two graph classes, \emph{grounded L}-graphs and \emph{stabbable grid intersection} graphs. An L-shape is made by joining the bottom end-point of a vertical ($\vert$) segment to the left end-point of a horizontal ($-$) segment. The top end-point of the vertical segment is known as the {\em anchor} of the L-shape. Grounded L-graphs are the intersection graphs of L-shapes such that all the L-shapes' anchors lie on the same horizontal line. We show that recognizing grounded L-graphs is NP-complete. This answers an open question asked by Jel{\'\i}nek \& T{\"o}pfer (Electron. J. Comb., 2019). Grid intersection graphs are the intersection graphs of axis-parallel line segments in which two vertical (similarly, two horizontal) segments cannot intersect. We say that a (not necessarily axis-parallel) straight line $\ell$ stabs a segment $s$, if $s$ intersects $\ell$. A graph $G$ is a stabbable grid intersection graph ($StabGIG$) if there is a grid intersection representation of $G$ in which the same line stabs all its segments. We show that recognizing $StabGIG$ graphs is $NP$-complete, even on a restricted class of graphs. This answers an open question asked by Chaplick \etal (\textsc{O}rder, 2018).

==> trash.tex <==

% \subsection{The proofs}

% We need to prove that $G$ is a yes-instance of {\sc PHPC} if and only if $\apexgraph{G}$ is a yes-instance of {\sc StabGIGRec}. We start with the backward direction.

% \begin{proposition}
% If $\apexgraph{G}$ is a $\StabGIG$, then $G$ is a yes-instance of {\sc PHPC}.
% \label{prop:backward}
% \end{proposition}

% \begin{proof}
% First, we show that if $\apexgraph{G}$ is a $\StabGIG$, then $\apexgraph{G}$ is a 1-string graph. To this end, it is sufficient to note that each segment in a grid representation of $\apexgraph{G}$ is a 1-string, and that two segments that intersect without crossing (because an enpoint of one segment lies on the second segment) may be easily transformed into two crossing segments.
% %Let $\mathcal{R}$ be a stabbable grid intersection representation of $\apexgraph{G}$. For every edge $e=uv$ of $\apexgraph{G}$, let $s_u$ and $s_v$ denote the segments in $\mathcal{R}$ corresponding to $u$ and $v$, respectively. Since $s_u$ and $s_v$ are of different orientations, they intersect at exactly one point. Now suppose, $s_u$ and $s_v$ do not cross each other. Then either $s_u$ contains one end-point of $s_v$ or vice versa. Without loss of generality, assume $s_u$ contains one end-point of $s_v$. Then observe that it is possible to elongate $s_v$ slightly so that the $s_v$ and $s_u$ cross each other and no new intersection point is formed. By performing the above operation (possibly) for all edges of $\apexgraph{G}$, it is possible to convert $\mathcal{R}$ into a $1$-String representation $\mathcal{R}'$ of $\apexgraph{G}$. Therefore, $\apexgraph{G}\in \OneString$. 
% Now, using Proposition~\ref{prop:yes-instance}, we deduce that $G$ is a yes-instance of {\sc PHPC}.
%  \end{proof}



% \begin{figure}
% 	\centering
% 	\scalebox{0.8}{
% 		\begin{tabular}{ccc}
% 			\rotatebox{90}{
% 				\begin{tikzpicture}
				
% 				\draw[densely dotted] (-2,0) -- (10.5,0);
% 				\def\A{4,0}
% 				\def\B{3,0}
% 				\def\C{2,0}
% 				\def\D{1,0}
% 				\def\E{0,0}
% 				\def\F{5,0}
% 				\def\G{6,0}
% 				\def\H{7,0}
% 				\def\J{4,-3}
% 				\def\K{8,0}
% 				\def\L{9,0}
% 				\renewcommand{\vertexset}{(a,\A,blue!60!white,,,blue!60!white),(b,\B,blue!60!white,,,blue!60!white),(c,\C,blue!60!white,,,blue!60!white),(d,\D,blue!60!white,,,blue!60!white),(e,\E,blue!60!white,,,blue!60!white),(f,\F,blue!60!white,,,blue!60!white),(g,\G,blue!60!white,,,blue!60!white),(h,\H,blue!60!white,,,blue!60!white),(j,\J,white,,,white),(k,\K,blue!60!white,,,blue!60!white),(l,\L,blue!60!white,,,blue!60!white)}
				
% 				\renewcommand{\edgeset}{(a,b,,,-0.5),(c,d,,,-0.5),(d,e,,,-0.5),(c,e,,,-1),(a,c,,,0.4),(a,d,,,0.7),(f,d,,,1.1),(g,d,,,1.6),(h,f,,,-0.4),(h,a,,,-0.8),(l,h,,,-0.4),(k,g,,,1),(l,a,,,-1.6),(l,k,,,0.5),(h,k,,,-0.5),(g,h,,,-0.5)}
				
% 				\renewcommand{\defradius}{0.07}
				
% 				\drawgraph
				
% 				\draw (1,0) .. controls (1,-1) .. (0,-1) .. controls (-1,-1) .. (-1,0) .. controls (-1,1) .. (1,1) .. controls (3,1) .. (3,0);
				
% 				\draw (6,0) .. controls (6,-1.5) .. (2,-1.5) .. controls (-1.5,-1.5) .. (-1.5,0) .. controls (-1.5,1.5) .. (1,1.5) .. controls (4,1.5) .. (4,0);
				
% 				\draw (4,0) .. controls (4,1.5) .. (6.5,1.5) .. controls (10,1.5) .. (10,0.25) .. controls (10,-1) .. (8.75,-1) .. controls (8,-1) .. (8,0);
				
% 				\node[left] at (-0.1,0) {\rotatebox{270} {\large $v_1$}};
% 				\node[left] at (0.9,-0.2) {\rotatebox{270} {\large $v_2$}};
% 				\node[right] at (2,0.2) {\rotatebox{270} {\large $v_3$}};
% 				\node[right] at (3,0) {\rotatebox{270} {\large $v_4$}};
% 				\node[right] at (4.1,0) {\rotatebox{270} {\large $v_5$}};
% 				\node[right] at (5.1,0) {\rotatebox{270} {\large $v_6$}};
% 				\node[right] at (6.1,0) {\rotatebox{270} {\large $v_7$}};
% 				\node[right] at (7.1,0) {\rotatebox{270} {\large $v_8$}};
% 				\node[right] at (8.1,0) {\rotatebox{270} {\large $v_9$}};
% 				\node[right] at (9.1,0) {\rotatebox{270} {\large $v_{10}$}};
% 				\end{tikzpicture}} & 
%     \rotatebox{90}{\begin{tikzpicture}
				
% 				\draw[densely dotted] (-2,0) -- (10.5,0);
% 				\def\A{4,0}
% 				\def\B{3,0}
% 				\def\C{2,0}
% 				\def\D{1,0}
% 				\def\E{0,0}
% 				\def\F{5,0}
% 				\def\G{6,0}
% 				\def\H{7,0}
% 				\def\J{4,-3}
% 				\def\K{8,0}
% 				\def\L{9,0}
% 				\renewcommand{\vertexset}{(a,\A,blue!60!white,,,blue!60!white),(b,\B,blue!60!white,,,blue!60!white),(c,\C,blue!60!white,,,blue!60!white),(d,\D,blue!60!white,,,blue!60!white),(e,\E,blue!60!white,,,blue!60!white),(f,\F,blue!60!white,,,blue!60!white),(g,\G,blue!60!white,,,blue!60!white),(h,\H,blue!60!white,,,blue!60!white),(j,\J,white,,,white),(k,\K,blue!60!white,,,blue!60!white),(l,\L,blue!60!white,,,blue!60!white)}
				
% 				\renewcommand{\edgeset}{(a,b,,,-0.5,dashed),(c,d,,,-0.5,dashed),(d,e,,,-0.5,dashed),(c,e,,,-1,dashed),(a,c,,,0.4,dashed),(a,d,,,0.7,dashed),(f,d,,,1.1,dashed),(g,d,,,1.6,dashed),(h,f,,,-0.4,dashed),(h,a,,,-0.8,dashed),(l,h,,,-0.4,dashed),(k,g,,,1,dashed),(l,a,,,-1.6,dashed),(l,k,,,0.5,dashed),(h,k,,,-0.5,dashed),(g,h,,,-0.5,dashed)}
				
% 				\renewcommand{\defradius}{0.07}

               	
    
% 				\drawgraph
				
% 				\draw[dashed] (1,0) .. controls (1,-1) .. (0,-1) .. controls (-1,-1) .. (-1,0) .. controls (-1,1) .. (1,1) .. controls (3,1) .. (3,0);
				
% 				\draw[dashed] (6,0) .. controls (6,-1.5) .. (2,-1.5) .. controls (-1.5,-1.5) .. (-1.5,0) .. controls (-1.5,1.5) .. (1,1.5) .. controls (4,1.5) .. (4,0);
				
% 				\draw[dashed] (4,0) .. controls (4,1.5) .. (6.5,1.5) .. controls (10,1.5) .. (10,0.25) .. controls (10,-1) .. (8.75,-1) .. controls (8,-1) .. (8,0);
				
% 				\node[left] at (-0.1,0) {\rotatebox{270} {\large $v_1$}};
% 				\node[left] at (0.9,-0.2) {\rotatebox{270} {\large $v_2$}};
% 				\node[right] at (2,0.2) {\rotatebox{270} {\large $v_3$}};
% 				\node[right] at (3,0) {\rotatebox{270} {\large $v_4$}};
% 				\node[right] at (4.1,0) {\rotatebox{270} {\large $v_5$}};
% 				\node[right] at (5.1,0) {\rotatebox{270} {\large $v_6$}};
% 				\node[right] at (6.1,0) {\rotatebox{270} {\large $v_7$}};
% 				\node[right] at (7.1,0) {\rotatebox{270} {\large $v_8$}};
% 				\node[right] at (8.1,0) {\rotatebox{270} {\large $v_9$}};
% 				\node[right] at (9.1,0) {\rotatebox{270} {\large $v_{10}$}};



    
% 				\end{tikzpicture}}
    
%     % \rotatebox{90}{\begin{tikzpicture}
				
% 				% \draw[densely dotted] (0,0) -- (7,0);
				
% 				% \def\A{4,0}
% 				% \def\B{3,0}
% 				% \def\C{2,0}
% 				% \def\D{1,0}
% 				% \def\E{0,0}
% 				% \def\F{5,0}
% 				% \def\G{6,0}
% 				% \def\H{7,0}
% 				% \def\J{4,-3}
				
% 				% \renewcommand{\vertexset}{(a,\A,blue!60!white,,,blue!60!white),(b,\B,blue!60!white,,,blue!60!white),(c,\C,blue!60!white,,,blue!60!white),(d,\D,blue!60!white,,,blue!60!white),(e,\E,blue!60!white,,,blue!60!white),(f,\F,blue!60!white,,,blue!60!white),(g,\G,blue!60!white,,,blue!60!white),(h,\H,blue!60!white,,,blue!60!white),(j,\J,white,,,white)}
				
% 				% \renewcommand{\edgeset}{(c,d,,,-0.5),(d,e,,,-0.5),(c,e,,,-1),(a,d,,,0.5),(f,d,,,0.8), (g,d,,,1), (h,f,,,-0.5),(h,a,,,-0.8)}
				
% 				% \renewcommand{\defradius}{0.07}
				
% 				% \drawgraph
				
%     %                 \draw (1,0) .. controls (1,-1) .. (0,-1) .. controls (-1,-1) .. (-1,0) .. controls (-1,1) .. (1,1) .. controls (3,1) .. (3,0);				
				
%     %                 \draw (6,0) .. controls (6,-1.5) .. (2,-1.5) .. controls (-1.5,-1.5) .. (-1.5,0) .. controls (-1.5,1.5) .. (1,1.5) .. controls (4,1.5) .. (4,0);
				
% 				% \filldraw[magenta!70!black] (0.825,0.25) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (0.625,0.37) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (0.4,0.37) circle (0.05cm);
				
% 				% \filldraw[magenta!70!black] (1.15,0.25) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (1.35,0.37) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (1.53,0.4) circle (0.05cm);
				
% 				% \filldraw[magenta!70!black] (0.625,0.7) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (1.35,0.7) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (1,0.75) circle (0.05cm);
				
% 				% \filldraw[magenta!70!black] (1,1) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (-1,0) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (0,-1) circle (0.05cm);
				
% 				% \filldraw[magenta!70!black] (1,1.5) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (-1.5,0) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (2,-1.5) circle (0.05cm);
				
% 				% \filldraw[magenta!70!black] (2.75,-0.375) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (3,-0.35) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (3.25,-0.32) circle (0.05cm);
				
% 				% \filldraw[magenta!70!black] (3.45,-0.575) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (3.7,-0.555) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (3.95,-0.49) circle (0.05cm);
				
% 				% \filldraw[magenta!70!black] (4.15,-0.72) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (4.4,-0.67) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (4.65,-0.62) circle (0.05cm);
				
% 				% \filldraw[magenta!70!black] (5.25,0.22) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (5.5,0.3) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (5.75,0.38) circle (0.05cm);
				
% 				% \filldraw[magenta!70!black] (4.75,0.5) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (5,0.575) circle (0.05cm);
% 				% \filldraw[magenta!70!black] (5.25,0.6) circle (0.05cm);
				
				
				
% 				% \node[left] at (-0.1,0) {\rotatebox{270} {\large $v_1$}};
% 				% \node[left] at (0.9,-0.2) {\rotatebox{270} {\large $v_2$}};
% 				% \node[right] at (2,0.2) {\rotatebox{270} {\large $v_3$}};
% 				% \node[right] at (3,0.2) {\rotatebox{270} {\large $v_4$}};
% 				% \node[right] at (4.1,0) {\rotatebox{270} {\large $v_5$}};
% 				% \node[right] at (5.1,0) {\rotatebox{270} {\large $v_6$}};
% 				% \node[right] at (6.1,0) {\rotatebox{270} {\large $v_7$}};
% 				% \node[right] at (7.1,0) {\rotatebox{270} {\large $v_8$}};
% 				% \end{tikzpicture}} 
%                     & 
                    
%                     \rotatebox{90}{\begin{tikzpicture}
				
% 				\draw[densely dotted] (-2,0) -- (10.5,0);
% 				\def\A{4,0}
% 				\def\B{3,0}
% 				\def\C{2,0}
% 				\def\D{1,0}
% 				\def\E{0,0}
% 				\def\F{5,0}
% 				\def\G{6,0}
% 				\def\H{7,0}
% 				% \def\J{4,-3}
% 				\def\K{8,0}
% 				\def\L{9,0}
%                     \def\AP{4,-2.8}
% 				\renewcommand{\vertexset}{(ap,\AP,magenta!70!black,0.2,,magenta!70!black),(a,\A,blue!60!white,,,blue!60!white),(b,\B,blue!60!white,,,blue!60!white),(c,\C,blue!60!white,,,blue!60!white),(d,\D,blue!60!white,,,blue!60!white),(e,\E,blue!60!white,,,blue!60!white),(f,\F,blue!60!white,,,blue!60!white),(g,\G,blue!60!white,,,blue!60!white),(h,\H,blue!60!white,,,blue!60!white),(k,\K,blue!60!white,,,blue!60!white),(l,\L,blue!60!white,,,blue!60!white)}
				
% 				\renewcommand{\edgeset}{(ap,l,gray,,-0.5),(ap,k,gray,,-0.5),(ap,h,gray,,-0.5),(ap,g,gray,,-0.5),(ap,f,gray,,-0.5),(ap,a,gray,,-0.5),(ap,b,gray,,-0.3),(ap,c,gray,,0.35),(ap,d,gray,,0.5),(ap,e,gray,,0.5),(a,b,,,-0.5,dashed),(c,d,,,-0.5,dashed),(d,e,,,-0.5,dashed),(c,e,,,-1,dashed),(a,c,,,0.4,dashed),(a,d,,,0.7,dashed),(f,d,,,1.1,dashed),(g,d,,,1.6,dashed),(h,f,,,-0.4,dashed),(h,a,,,-0.8,dashed),(l,h,,,-0.4,dashed),(k,g,,,1,dashed),(l,a,,,-1.6,dashed),(l,k,,,0.5,dashed),(h,k,,,-0.5,dashed),(g,h,,,-0.5,dashed)}
				
% 				\renewcommand{\defradius}{0.07}

               	
    
% 				\drawgraph
				
% 				\draw[dashed] (1,0) .. controls (1,-1) .. (0,-1) .. controls (-1,-1) .. (-1,0) .. controls (-1,1) .. (1,1) .. controls (3,1) .. (3,0);
				
% 				\draw[dashed] (6,0) .. controls (6,-1.5) .. (2,-1.5) .. controls (-1.5,-1.5) .. (-1.5,0) .. controls (-1.5,1.5) .. (1,1.5) .. controls (4,1.5) .. (4,0);
				
% 				\draw[dashed] (4,0) .. controls (4,1.5) .. (6.5,1.5) .. controls (10,1.5) .. (10,0.25) .. controls (10,-1) .. (8.75,-1) .. controls (8,-1) .. (8,0);
				
% 				\node[left] at (-0.1,0) {\rotatebox{270} {\large $v_1$}};
% 				\node[left] at (0.9,-0.2) {\rotatebox{270} {\large $v_2$}};
% 				\node[right] at (2,0.2) {\rotatebox{270} {\large $v_3$}};
% 				\node[right] at (3,0) {\rotatebox{270} {\large $v_4$}};
% 				\node[right] at (4.1,0) {\rotatebox{270} {\large $v_5$}};
% 				\node[right] at (5.1,0) {\rotatebox{270} {\large $v_6$}};
% 				\node[right] at (6.1,0) {\rotatebox{270} {\large $v_7$}};
% 				\node[right] at (7.1,0) {\rotatebox{270} {\large $v_8$}};
% 				\node[right] at (8.1,0) {\rotatebox{270} {\large $v_9$}};
% 				\node[right] at (9.1,0) {\rotatebox{270} {\large $v_{10}$}};



    
% 				\end{tikzpicture}}\\
% 			(a) & (b) & (c)
   
% 	\end{tabular}}
% 	\caption{
%  % \rt{A general remark concerning figures: they use colors, which is very good, but does that means that you wish to pay the "color" supplement for the publication? I never do it, this is why my figures are always in black and white.}  
%  (a) An example graph $G$ which is a yes-instance of {\sc PHPC}. (b) Each edge of the graph is replaced by a path of length $k+1$ where $k\geq 7$. A dashed curve indicates a path of length $k$. (c) The apex graph $\apexgraph{G}$ constructed by adding one extra vertex in $\subdivide{G}$.}\label{fig:representation}
% \end{figure}

% \begin{figure}
%     \centering
    

% \rotatebox{90}{\begin{tikzpicture}
				
% 				\draw[densely dotted] (-2,0) -- (10.5,0);
% 				\def\A{4,0}
% 				\def\B{3,0}
% 				\def\C{2,0}
% 				\def\D{1,0}
% 				\def\E{0,0}
% 				\def\F{5,0}
% 				\def\G{6,0}
% 				\def\H{7,0}
% 				\def\K{8,0}
% 				\def\L{9,0}
                    
%                     \def\AP{4,-2.8}
                    
% 				\renewcommand{\vertexset}{(ap,\AP,magenta!70!black,0.2,,magenta!70!black),(a,\A,blue!60!white,,,blue!60!white),(b,\B,blue!60!white,,,blue!60!white),(c,\C,blue!60!white,,,blue!60!white),(d,\D,blue!60!white,,,blue!60!white),(e,\E,blue!60!white,,,blue!60!white),(f,\F,blue!60!white,,,blue!60!white),(g,\G,blue!60!white,,,blue!60!white),(h,\H,blue!60!white,,,blue!60!white),(k,\K,blue!60!white,,,blue!60!white),(l,\L,blue!60!white,,,blue!60!white)}
				
% 				\renewcommand{\edgeset}{(ap,l,gray,,-0.5),(ap,k,gray,,-0.5),(ap,h,gray,,-0.5),(ap,g,gray,,-0.5),(ap,f,gray,,-0.5),(ap,a,gray,,-0.5),(ap,b,gray,,-0.3),(ap,c,gray,,0.35),(ap,d,gray,,0.5),(ap,e,gray,,0.5),(a,b,,,-0.5),(c,d,,,-0.5),(d,e,,,-0.5),(c,e,,,-1),(a,c,,,0.4),(a,d,,,0.7),(f,d,,,1.1),(g,d,,,1.6),(h,f,,,-0.4),(h,a,,,-0.8),(l,h,,,-0.4),(k,g,,,1),(l,a,,,-1.6),(l,k,,,0.5),(h,k,,,-0.5),(g,h,,,-0.5)}
				
% 				\renewcommand{\defradius}{0.07}

               	
    
% 				\drawgraph
				
% 				\draw (1,0) .. controls (1,-1) .. (0,-1) .. controls (-1,-1) .. (-1,0) .. controls (-1,1) .. (1,1) .. controls (3,1) .. (3,0);
				
% 				\draw (6,0) .. controls (6,-1.5) .. (2,-1.5) .. controls (-1.5,-1.5) .. (-1.5,0) .. controls (-1.5,1.5) .. (1,1.5) .. controls (4,1.5) .. (4,0);
				
% 				\draw (4,0) .. controls (4,1.5) .. (6.5,1.5) .. controls (10,1.5) .. (10,0.25) .. controls (10,-1) .. (8.75,-1) .. controls (8,-1) .. (8,0);
				
% 				\node[left] at (-0.1,0) {\rotatebox{270} {\large $v_1$}};
% 				\node[left] at (0.9,-0.2) {\rotatebox{270} {\large $v_2$}};
% 				\node[right] at (2,0.2) {\rotatebox{270} {\large $v_3$}};
% 				\node[right] at (3,0) {\rotatebox{270} {\large $v_4$}};
% 				\node[right] at (4.1,0) {\rotatebox{270} {\large $v_5$}};
% 				\node[right] at (5.1,0) {\rotatebox{270} {\large $v_6$}};
% 				\node[right] at (6.1,0) {\rotatebox{270} {\large $v_7$}};
% 				\node[right] at (7.1,0) {\rotatebox{270} {\large $v_8$}};
% 				\node[right] at (8.1,0) {\rotatebox{270} {\large $v_9$}};
% 				\node[right] at (9.1,0) {\rotatebox{270} {\large $v_{10}$}};

%                 \filldraw[cyan] (10,0) circle (3pt);
%                 \filldraw[cyan] (-1,0) circle (3pt);
%                 \filldraw[cyan] (-1.5,0) circle (3pt);

%                 \filldraw[magenta] (2,1) circle (1.2pt); \filldraw[magenta] (1.5,1) circle (1.2pt); \filldraw[magenta] (1,1) circle (1.2pt);

%                 \filldraw[magenta] (2,1.5) circle (1.2pt); \filldraw[magenta] (1.5,1.5) circle (1.2pt); \filldraw[magenta] (1,1.5) circle (1.2pt);

%                 \filldraw[magenta] (7,1.5) circle (1.2pt); \filldraw[magenta] (6.5,1.5) circle (1.2pt); \filldraw[magenta] (6,1.5) circle (1.2pt);

%                 \filldraw[magenta] (7,1.18) circle (1.2pt); \filldraw[magenta] (6.5,1.21) circle (1.2pt); \filldraw[magenta] (6,1.18) circle (1.2pt);

%                 \filldraw[magenta] (2.2,-1.5) circle (1.2pt); \filldraw[magenta] (1.7,-1.5) circle (1.2pt); \filldraw[magenta] (1,-1.5) circle (1.2pt);

%                 \filldraw[magenta] (0.5,-1) circle (1.2pt); \filldraw[magenta] (0,-1) circle (1.2pt); \filldraw[magenta] (-0.5,-1) circle (1.2pt);

%                 \filldraw[magenta] (9.5,-0.975) circle (1.2pt); \filldraw[magenta] (9,-1) circle (1.2pt); \filldraw[magenta] (8.5,-1) circle (1.2pt);

%                 \filldraw[magenta] (8.3,-0.34) circle (1.2pt); \filldraw[magenta] (8.4,-0.37) circle (1.2pt); \filldraw[magenta] (8.55,-0.375) circle (1.2pt);

                
%                 \filldraw[magenta] (3,-0.315) circle (1.2pt); \filldraw[magenta] (2.8,-0.3) circle (1.2pt); \filldraw[magenta] (3.35,-0.275) circle (1.2pt);

%                 \filldraw[magenta] (3,-0.827) circle (1.2pt); \filldraw[magenta] (2.8,-0.825) circle (1.2pt); \filldraw[magenta] (3.35,-0.825) circle (1.2pt);

%                 \filldraw[magenta] (3,-1.17) circle (1.2pt); \filldraw[magenta] (2.8,-1.14) circle (1.2pt); \filldraw[magenta] (3.35,-1.21) circle (1.2pt);

%                 \filldraw[magenta] (3,-0.5) circle (1.2pt); \filldraw[magenta] (2.8,-0.525) circle (1.2pt); \filldraw[magenta] (3.4,-0.39) circle (1.2pt);
                
%                 \filldraw[magenta] (8,0.32) circle (1.2pt); \filldraw[magenta] (7.7,0.28) circle (1.2pt); \filldraw[magenta] (8.25,0.3) circle (1.2pt);

%                 \filldraw[magenta] (6,0.32) circle (1.2pt); \filldraw[magenta] (5.7,0.28) circle (1.2pt); \filldraw[magenta] (6.25,0.3) circle (1.2pt);

%                 \filldraw[magenta] (6,0.555) circle (1.2pt); \filldraw[magenta] (5.7,0.6) circle (1.2pt); \filldraw[magenta] (6.25,0.5) circle (1.2pt);
                
%                 \filldraw[magenta] (7.3,-0.34) circle (1.2pt); \filldraw[magenta] (7.4,-0.37) circle (1.2pt); \filldraw[magenta] (7.55,-0.375) circle (1.2pt);

%                 \filldraw[magenta] (6.8,-0.74) circle (1.2pt); \filldraw[magenta] (6.9,-0.77) circle (1.2pt); \filldraw[magenta] (7.05,-0.775) circle (1.2pt);
                
%                 \filldraw[magenta] (6.3,-0.34) circle (1.2pt); \filldraw[magenta] (6.4,-0.37) circle (1.2pt); \filldraw[magenta] (6.55,-0.375) circle (1.2pt);


%                 \filldraw[magenta] (0.7,0.34) circle (1.2pt); \filldraw[magenta] (0.4,0.37) circle (1.2pt); \filldraw[magenta] (0.55,0.375) circle (1.2pt);

%                 \filldraw[magenta] (1.2,0.74) circle (1.2pt); \filldraw[magenta] (0.9,0.77) circle (1.2pt); \filldraw[magenta] (1.05,0.775) circle (1.2pt);

%                 \filldraw[magenta] (1.7,0.34) circle (1.2pt); \filldraw[magenta] (1.4,0.37) circle (1.2pt); \filldraw[magenta] (1.55,0.375) circle (1.2pt);

%                 \filldraw[magenta] (3.7,0.34) circle (1.2pt); \filldraw[magenta] (3.4,0.37) circle (1.2pt); \filldraw[magenta] (3.55,0.375) circle (1.2pt);
                
% 			\end{tikzpicture}}
%     \caption{The graph $\apexgraphthree{H}$ constructed from the the graph shown in Figure~\ref{fig:representation}(a). The bigger vertices are introduced in $\apexgraphthree{H}$.  The graph $\apexgraphseven{G}$ is then obtained from $\apexgraphthree{H}$ by further subdividing with 4 vertices each edge $v_iv_j$. \rt{Now that the colors are present in the text, I understand that we will pay the "colors" option for the publication. I need to say that I do not have the founding for doing that ...} \textcolor{blue}{D: Perhaps we can take this approach. For the arxiv version, we can put the colors. For the publications that would require money, we will change back the colors to black and white. (I do not have the funding for it too.) In our previous paper, there were colors too, without any extra payment.} \rt{I agree with this. But if you put the colors in the text, that means you will have to change not only the figures but also the text.} Ah, Sorry that I did not understand the issue completely before. I changed the texts. Illustration of the reduction. }
%     \label{fig:proof-illustration}
% \end{figure}

% % \begin{figure}

% % 	\scalebox{0.4}{

                
% % \begin{tikzpicture}

% %     \draw[thick,magenta!70!black] (0,0) -- (0,16);

% %     \draw[dotted] (-13,-13) -- (16,16);
    
% %     \coordinate (le1) at (-1,0); \coordinate (re1) at (26,0);

% %     \coordinate (le2) at (-2,1); \coordinate (re2) at (25,1);
% %     \coordinate (le3) at (-3,2); \coordinate (re3) at (24,2);
    
% %     \coordinate (le4) at (-4,3); \coordinate (re4) at (23,3);

    
% %     \coordinate (le5) at (-5,4); \coordinate (re5) at (22,4);

    
% %     \coordinate (le6) at (-6,5); \coordinate (re6) at (21,5);

    
% %     \coordinate (le7) at (-7,6); \coordinate (re7) at (20,6);


% %     \coordinate (le8) at (-8,7); \coordinate (re8) at (19,7);

% %     \coordinate (le9) at (-9,8); \coordinate (re9) at (18,8);

% %     \coordinate (le10) at (-10,9); \coordinate (re10) at (17,9);

% %     \coordinate (le11) at (-11,10); \coordinate (re11) at (16,10);
    
% %     \coordinate (le12) at (-12,11); \coordinate (re12) at (15,11);

% %     \coordinate (le13) at (-13,12); \coordinate (re13) at (14,12);


% %     \draw[cyan] (le1) -- (re1); \draw[cyan] (le2) -- (re2); \draw (le3) -- (re3); \draw (le4) -- (re4); \draw (le5) -- (re5); \draw (le6) -- (re6); \draw (le7) -- (re7); \draw (le8) -- (re8); \draw (le9) -- (re9); \draw (le10) -- (re10); \draw (le11) -- (re11); \draw (le12) -- (re12); \draw[cyan] (le13) -- (re13); 

% %     \draw[magenta] (le13) -- (-13,-13); \draw[magenta] (-6.2,6) -- (-6.2,-13) ; \draw[magenta] (-13.2,-13) -- (-6,-13) ;

% %     \draw[magenta] (le12) -- (-12,-12); \draw[magenta] (-6.6,6) -- (-6.6,-12) ; \draw[magenta] (-12.2,-12) -- (-6.4,-12) ;*

    
% %     \draw[magenta] (le12) -- (-12,-12); \draw[magenta] (-6.6,6) -- (-6.6,-12) ; \draw[magenta] (-12.2,-12) -- (-6.4,-12) ;
    
% % \end{tikzpicture}
        
% %             }
% % 	\caption{A partial stabbable grid intersection representation of $\apexgraphthree{H}$. \textcolor{blue}{I think it would be better to give representation of only few segments in the left and right side. A complete representation of $\apexgraph{G}$ would be cluttered and therefore may not be very helpful. What do you think ?} \rt{ I think that finally a much smaller example would have been easier to deal with. Taking only the bottom part of it (from $v_5$ to $v_{10}$) would probably be a better idea, but would require to modify many things, and I don't know if this is easy or not with tikZ (?)}
% % 	\textcolor{magenta}{In all cases, I think we should give the detail of the representation of an edge (I think we need a figure like the next, handmade, figure I included in the paper: Figure 9). Then, two cases: either you can cut the example in order to have a much smaller one that we can represent entirely; or you cannot cut it, and then we choose to represent only a part of it, for instance the one I suggested above, or even a smaller one, but which has all types of edges.}
% % \rt{I also note that the colours of the segments are not exactly the colours of the vertices they represent (this is the case only for the new vertices in H). }
% % \textcolor{magenta}{And for the further subdivision I wrote yesterday, I suggest something like the second figure (next page, Figure 10)} 

% % I agree
% % }



% %  \label{fig:proof-illustrate}
% % \end{figure}







%  \begin{figure}[t!]
%  \centering
%  \includegraphics[scale=0.5]{fig-const-2-crop.pdf}
%  \caption{Replacement of $\curve{u_e^2}$ with a path of length $2h+1$. In this figure, $h=2$. }
%  \end{figure}
 

% The forward direction is presented below, for $k\geq 7$. 

% % The notation $[n]$ stands for $\{1, 2, \ldots, n\}$.

% % \textcolor{blue}{I have already defined it once. Do we need to recall it here ?}

% \begin{proposition}\label{prop:forward}
% Let $k\geq 7$ be an odd integer. If $G$ is a yes-instance of {\sc PHPC}, then $\apexgraph{G}$ is a $\StabGIG$. 
% \end{proposition}

% \begin{proof} We prove~\autoref{prop:forward} for graphs with $k=7$ (\ie, of girth $g=10$), and we will observe later that our proof works for all values of $g\geq 10$, where $g$ is a fixed constant.

% Let $V(G)=\{v_1,v_2,\ldots,v_n\}$. We start with a plane drawing of $G$, \ie, a drawing of $G$ in the plane, in which the vertices are points and the edges are strings (that is, simple curves). Then we modify the drawing in a step-by-step manner to end with a $\StabGIG$ representation of $\apexgraphseven{G}$. Let us now provide an overview of these steps.

% \begin{enumerate}[label=(\alph*)]

%     \item \label{enum:step1auergleisner} Consider a drawing of $G$ in the plane in which the vertex $v_i$ (for every $i\in[n]$) has the Cartesian coordinate $(0,i-1)$, each edge of $G$ crosses the y-axis (the line $x=0)$ at most once, and no edge of $G$ crosses the y-axis between $y=0$ and $y=n-1$. (Auer \& Glei{\ss}ner~\cite{auer2011} show that such a drawing exists for every graph that is a yes-instance of {\sc PHPC}.)
    
%     \item \label{enum:step2creationofH} In this drawing, though no edge of $G$ crosses $((0,0),(0,n-1))$, there might be edges of $G$ that cross the y-axis below $y=0$ or above $y=n-1$. We place `new' vertices on those intersection points of the edges with the y-axis, to create a new graph $H$. Let $n_H$ be the number of vertices in $H$.
    
%     \item \label{enum:step3propertiesofH} The graph $H$ has some nice properties. Firstly, $n\leq n_H\leq 4n$. Secondly, $H$ is a subdivision of $G$. As subdivision does not affect planarity, $H$ is also planar. Thirdly, the drawing of $H$ ensures that no edge of $H$ crosses the y-axis. We fix the line $y=x$ as our stab line $\ell$ (recall that $\ell$ does need not to be axis-parallel), and use the current plane drawing of $H$ to devise a $\StabGIG$ representation of the graph $\apexgraphthree{H}$. (The graph $\apexgraphthree{H}$ is obtained as described in the previous section, by considering $P=H$ and $k=3$.) Note that the graph $\apexgraphseven{G}$ is obtained from $\apexgraphthree{H}$ by further subdividing some of its edges. %passing through the origin at a $45\degree$ angle, namely $y=x$. We will show that $\ell$ stabs all the segments of $\apexgraph{H}$.
    
%     \item \label{enum:step4representationofH} In the $\StabGIG$ representation of $\apexgraphthree{H}$, the apex segment of $\apexgraphthree{H}$ is represented by a long vertical segment coinciding with the y-axis. The $n_H$ original vertices of $\apexgraphthree{H}$ are represented by $n_H$ horizontal segments, each one crossing the y-axis at the same point as its corresponding vertex in the plane representation of $H$. Each edge $e=xy$ of $H$ (which is a string in the plane drawing of $H$) becomes a path with three intermediate vertices $u_e^1, u_e^2, u_e^3$ in $\apexgraphthree{H}$. These three vertices are represented as three segments that form a $\U$-shape or a $\Urev$-shape, whose two vertical segments appropriately intersect the vertical segments representing respectively $x$ and $y$. %is represented by a rectilinear piecewise linear curve with three pieces in $\apexgraphthree{H}$.%If we were allowed a large number of rectilinear pieces for each edge, then this construction is trivial, since every curve can be viewed as a series of infinitesimally small vertical and horizontal segments. Our proof formally justifies that this can always be done when the number of allowed rectilinear pieces is a fixed odd integer greater than or equal to three.

%     \item \label{enum:step5nontrivial} So far, our construction is similar to the construction in~\cite{chakraborty2022}. But now, we have to slightly deviate from it. For each edge $e$ of $H$, we need to very precisely and carefully describe the positions of the three segments corresponding to its three subdivision vertices $u^1_e, u^2_e, u^3_e$ in $\apexgraphthree{H}$, in such a way that all the three segments intersect the stab line $\ell$. This is the most novel and non-trivial part of our proof.
    
%     \item \label{enum:step6sevensubdiv} Finally, we need to convert $\apexgraphthree{H}$ to $\apexgraphseven{G}$. Note that $\apexgraphthree{H}\setminus\{a\}$ is a subdivision of $G$ in which each edge of $G$ is subdivided either 3 or 7 times. It is easy to add more segments to the $\StabGIG$ representation to ensure that all edges of $G$ are subdivided exactly $k$ times, for any odd number $k\geq 7$. Now, with the apex segment $((0,0),(0,n-1))$, we have a $\StabGIG$ representation of $\apexgraph{G}$.%After this shortening, the `new' vertices become subdivision vertices of $G$. It is easy to add more segments to the $\StabGIG$ representation to ensure that all edges of $G$ are subdivided exactly $k$ times, for any odd number $k\geq 7$.
    
%     %Note that $\apexgraphthree{H}\setminus\{a\}$ is a subdivision of $G$. So, all we need to do is ensure that $a$ is connected to the original vertices of $G$ only. Now the apex segment no longer intersects the horizontal segments corresponding to the `new' vertices, and we have a $\StabGIG$ representation of $\apexgraph{G}$. %Consequently, $\apexgraph{H}$ loses the edges between the apex vertex $a$ with the `new' vertices. Thus, $a$ is now only connected to the original vertices of $G$. Since $H$ was a subdivision of $G$, this modified graph is $\apexgraph{G}$.
%     %\item Our stab line $\ell$ (not part of the construction) will be the line passing through the origin at a $45\degree$ angle, namely $y=x$. We will show that $\ell$ stabs all the segments of $\apexgraph{H}$.
% \end{enumerate}

% Now we commence with the formal proof of~\autoref{prop:forward}. Let us start with~\autoref{enum:step1auergleisner}. Since $G$ is a yes-instance of {\sc PHPC}, according to Auer \& Glei{\ss}ner~\cite{auer2011}, the edge set $E(G)$ can be partitioned into three sets $\Eleftedge(G)$, $\Erightedge(G)$, and $\Ecrossedge(G)$, such that $G$ admits a plane drawing satisfying the following properties.
% \begin{itemize}
%     \item For every $i\in[n]$, the vertex $v_i$ has the Cartesian coordinate $(0,i-1)$.
%     \item Every edge $e\in\Eleftedge(G)$ lies in the half-plane $x\leq 0$.
%     \item Every edge $e\in\Erightedge(G)$ lies in the half-plane $x\geq 0$.
%     \item Every edge $e\in\Ecrossedge(G)$ crosses the line $x=0$ exactly once, at $(0,Y_e)$, where $Y_e<0$ or $Y_e>n-1$.
% \end{itemize}
% See~\autoref{fig:representation}(a) for a plane drawing which satisfies the above properties. We will be using this graph as a running example for our proof. Note that the above plane drawing crucially uses the fact that the line $x=0$ partitions the plane into two half-planes ($x\leq 0$ and $x\geq 0$). Now, let us move on to~\autoref{enum:step2creationofH}.
% %Note that the edge $(v_2,v_4)$ crosses the y-axis at the point $(0,-1)$, the edge $(v_5,v_7)$ crosses the y-axis at $(0,-2)$, and the edge $(v_5,v_9)$ crosses the y-axis at $(0,10)$.

% The construction of $H$ from $G$ is done as follows. For each edge $e=v_i,v_j\in\Ecrossedge(G)$, we add a `new' vertex $\newvert_e$ to the graph, represented by the point $(0,Y_e)$. Consequently, the edge $e=v_iv_j$ is replaced by two edges $v_i\newvert_e$ and $\newvert_ev_j$. One of those edges is in $\Eleftedge(H)$ and the other is in $\Erightedge(H)$. Therefore, the vertex $\newvert_e$ is a subdivision vertex of the edge $e$. More formally,
% \begin{align*}
%     V(H)&=V(G)\cup\{\newvert_e\mid e\in\Ecrossedge(G)\};\\
%     E(H)&=\Eleftedge(G)\cup\Erightedge(G)\cup\{(x,\newvert_e),(\newvert_e,y)\mid e=(x,y)\in\Ecrossedge(G)\}.
% \end{align*}
% What did this achieve for us? The graph $H$ has some nice properties, which we mentioned in~\autoref{enum:step3propertiesofH}, and will elaborate now.
% \begin{itemize}
%     \item $H$ is a subdivision of $G$. Edges of $\Eleftedge(G)$ and $\Erightedge(G)$ are retained as-is in $H$, and edges of $\Ecrossedge(G)$ are subdivided once.
%     \item $H$ is a planar graph. This is because $G$ is a planar graph, and subdivision does not affect planarity.
%     \item No edge of $H$ crosses the y-axis ($\Ecrossedge(H)=\emptyset$). This is a straightforward feature of our construction.
%     \item $n\leq n_H \leq 4n$, where $n_H=|V(H)|$. This is because $G$ has at most $3n$ edges (as $G$ is planar), and each edge of $G$ is subdivided at most once in $H$. Since $H$ also retains the vertices of $G$, $n_H \leq n+3n$.
% \end{itemize}
% %The graph $H$ has the properties that we require. 
% From $H$, we construct $\apexgraphthree{H}$, as described in Section~\ref{subsec:reduction2}. We first define the positions of the segments corresponding to the apex vertex of $\apexgraphthree{H}$ and the original vertices of $H$ in our $\StabGIG$ representation of $\apexgraphthree{H}$ (\autoref{enum:step4representationofH}). Note that the apex vertex in $\apexgraphthree{H}$ is called $a$, just as the apex vertex in $\apexgraph{G}$, since these vertices finally coincide in our construction. 

% The vertices with the minimum and maximum y-coordinates in $H$ are at $(0,Y_{\min})$ and $(0,Y_{\max})$, where
% \begin{align*}
% Y_{\min}&=\operatorname{min}\left(\{0\}\cup\{Y_e\mid e\in\Ecrossedge(G)\}\right);\\
% Y_{\max}&=\operatorname{max}\left(\{n-1\}\cup\{Y_e\mid e\in\Ecrossedge(G)\}\right).
% \end{align*}
% We may assume that $Y_{\min}=0$ and $Y_{\max}=n_H-1$, and that the other vertices of $H$ can be shifted accordingly so that their coordinates are $(0,0), (0,1), (0,2), \ldots, (0,n_H-1)$.\footnote{This can be done, for example, by shifting the x-axis downwards and making the gap between consecutive points as $1$.} Furthermore, the vertices are suitably renamed as $w_1, w_2, w_3, \ldots, w_{n_H}$ so that each $w_i$ has the coordinate $(0,i-1)$. Now let us set a nomenclature for the segments. For each vertex $x\in V(H)\cup\{a\}$, let $\curve{x}$ be its corresponding segment.
% \begin{align*}
%     &\text{The apex vertex $a$ of $\apexgraphthree{H}$:}&&\curve{a} = ((0,0),(0,n_H-1));\\
%     &\text{The original vertices of $H$:}&&\curve{w_i} = ((-i-0.1,i-1),(2n_H-i+0.1,i-1))\qquad\forall\,i\in[n_H].
% \end{align*}



% We fix the line $y=x$ as our stab line $\ell$ (recall that $\ell$ does not need to be axis-parallel). It is easy to see that all the segments described so far intersect the stab line \rt{stab line or stabbing line? we should use the same terminology everywhere}. This brings us to~\autoref{enum:step5nontrivial}, where we need to place the segments corresponding to the three subdivision vertices of $e$ for each edge $e$ of $H$.

% Let us consider edges of $\Eleftedge(H)$. Later, we will deal with edges of $\Erightedge(H)$. We will construct a set of intervals $\Ileft$ from $\Eleftedge(H)$ as follows. For each edge $e=(w_i,w_j)\in\Eleftedge(H)$ (where $i<j$), the set $\Ileft$ contains an open interval $(i-1,j-1)$. Thus, the number of intervals in $\Ileft$ is the number of edges in $\Eleftedge(H)$. Now, note that $\Ileft$ has the following interesting property.

% \begin{observation} \label{obs:bookthickness}
%     If two intervals of $\Ileft$ have an overlap (\ie, the intervals are not disjoint), then one of them must be contained in the other.
%     %Let $I_1\in\Ileft$ and $I_2\in\Ileft$ be two intervals. Then, exactly one of the following is true.
%     %\begin{itemize}
%         %\item $I_1$ and $I_2$ are disjoint.
%         %\item $I_1$ contains $I_2$, or $I_2$ contains $I_1$.
%     %\end{itemize}
% \end{observation}

% Observation~\ref{obs:bookthickness} is well known and easy to see; it is the basic underlying principle of \emph{book thickness} or \emph{book embeddings} of graphs (for a proof, see~\cite{bernhartkainen1979}). %Let us try to understand how this observation benefits us. It implies that if $(i_1,j_1)\in\Ileft$ and $(i_2,j_2)\in\Ileft$, then $i_1<i_2<j_1<j_2$ and $i_2<i_1<j_2<j_1$ are both impossible.
% We will use this observation crucially in our construction of the three subdivision segments for each edge $e$ of $\Eleftedge(H)$.

% Given an interval $I\in\Ileft$, let its \emph{depth}, denoted by $\level{I}$, be the number of intervals $I'\in\Eleftedge(H)$ such that $I\subseteq I'$. In other words, $\level{I}$ is the number of intervals that contain $I$ (including $I$ itself). Thus, $1\leq\level{I}\leq n_H-1$. Now we are ready to describe our construction.

% Fix $\varepsilon=0.01/n_H$. Let $e=(w_i,w_j)\in\Eleftedge(H)$ such that $i<j$. Let $I=(i-1,j-1)$ be the interval corresponding to $e$ in $\Ileft$. After the $3$-subdivision, the edge $e$ becomes the path $(w_i,u_e^1,u_e^2,u_e^2,w_j)$ in $\apexgraphthree{H}$. We already know the coordinates of the segments for $w_i$ and $w_j$. As for the other three segments, we define $\lefty_e$ and $\righty_e$ as follows.
% \begin{align*}
%     \lefty_e &= -j+\varepsilon\level{I};\\
%     \righty_e &= -i-\varepsilon\level{I}.
% \end{align*}
% Now, we are set to define the coordinates of the other three subdivision segments of $e$, which draw a $\U$-shape.
% \begin{align*}
%     \curve{u_e^3} &= \left((\lefty_e,j-1),(\lefty_e,\lefty_e)\right);\\
%     \curve{u_e^2} &= \left((\lefty_e,\lefty_e),(\righty_e,\lefty_e)\right);\\
%     \curve{u_e^1} &= \left((\righty_e,\lefty_e),(\righty_e,i-1)\right).
% \end{align*}
% %\begin{observation}
%     %The $3$ segments $\curve{u_e^3},\curve{u_e^2},\curve{u_e^1}$ lie on the boundary of an axis-parallel rectangle $R_e$, whose opposite corners are
%     %\begin{align*}
%         %\text{Top left: } &(\lefty_e,j-1);\\
%         %\text{Bottom right: } &(\righty_e,\lefty_e).
%     %\end{align*}
% %\end{observation}
% Before proving that the 3 segments do not intersect any segments apart from $w_i$, $w_j$, and each other, let us prove that all 3 segments intersect the stab line. Consider the point of intersection of $\curve{u_e^3}$ and $\curve{u_e^2}$, namely $(\lefty_e,\lefty_e)$. This point has the same x- and y-coordinate, and so it lies on the stab line $y=x$. Thus, all that remains to be shown is that $\curve{u_e^1}$ also intersects the stab line. Since $i\leq j-1$ and $\varepsilon\level{I}<0.01$, $$\lefty_e \leq \righty_e \leq i-1.$$ Hence, the point $(\righty_e,\righty_e)$ lies on the segment $\curve{u_e^1} = \left((\righty_e,\lefty_e),(\righty_e,i-1)\right)$, and on the stab line $y=x$ also.

% Now, we will show that for two edges $e=(w_i,w_j)$ (where $i<j$) and $e'=(w_{i'},w_{j'})$ (where $i'<j'$) of $\Eleftedge(H)$, the segments corresponding to the three subdivision vertices of $e$ do not intersect the segments corresponding to the three subdivision vertices of $e'$. Let their corresponding intervals in $\Ileft$ be $I$ and $I'$, respectively. Due to Observation~\ref{obs:bookthickness}, we have only two cases.
% \begin{enumerate}
%     \item \underline{Case 1: $I$ and $I'$ are disjoint.} Suppose that $i<j\leq i'<j'$ (the other sub-case, $i'<j'\leq i<j$, is similar). We have the following.
%     \begin{align*}
%         i < j&\leq i' < j'\\
%         -j' < -i'&\leq -j < -i\\
%         -j'+\varepsilon\level{I'}<-i'-\varepsilon\level{I'}&< -j+\varepsilon\level{I}<-i-\varepsilon\level{I} &&\text{(since $2\varepsilon\level{I'}<1\leq j'-i'$ and $2\varepsilon\level{I}<1\leq j-i$)}\\
%         \lefty_{e'} < \righty_{e'} &< \lefty_{e} < \righty_{e}
%     \end{align*}
    
%     Thus, the x-coordinate of each of the 3 subdivision segments of $e'$ is at most $\righty_{e'}$, and the x-coordinate of each of the 3 subdivision segments of $e$ is at least $\lefty_e$. This completes the proof of Case 1.
    
%     \item \underline{Case 2: One of $I$ or $I'$ contains the other.} Suppose that $I\subseteq I'$ (the other sub-case, $I'\subseteq I$, is similar). Then, note that $\level{I'}<\level{I}$. We have the following.
%     \begin{align*}
%         i' \leq i &< j \leq j' &&\text{(since $I\subseteq I'$)}\\
%         -j' \leq -j &< -i \leq -i'\\
%         -j' + \varepsilon\level{I'} < -j + \varepsilon\level{I} &< -i - \varepsilon\level{I} < -i' - \varepsilon\level{I'} &&\text{(since $\level{I'}<\level{I}$ and $2\varepsilon\level{I}<1\leq j-i$)}\\
%         \lefty_{e'}<\lefty_{e}&<\righty_{e}<\righty_{e'}
%     \end{align*}
%     Thus, the x-coordinate of $\curve{u_{e'}^3}$ (namely $\lefty_{e'}$) is less than the x-coordinate of each of the 3 subdivision segments of $e$, and the x-coordinate of $\curve{u_{e'}^1}$ (namely $\righty_{e'}$) is greater than the x-coordinate of each of the 3 subdivision segments of $e$. Finally, the y-coordinate of $\curve{u_{e'}^2}$ (namely $\lefty_{e'}$) is less than the y-coordinate of each of the 3 subdivision segments of $e$. This completes the proof of Case 2.
% \end{enumerate}

% This completes the construction of the $\StabGIG$ representation for the subgraph of $\apexgraphthree{H}$ induced by the original vertices of $H$, the apex vertex $a$ and the subdivision vertices located in the left half-plane. For the vertices and edges located in the right half-plane, the construction is similar but replaces the $\U$-shapes by $\Urev$-shapes. The correctness of our construction follows from Cases 1 and 2 above.
% \bigskip


%  In order to conclude our proof of~\autoref{prop:forward}, we need according to~\autoref{enum:step6sevensubdiv}: (1) to convert the $\StabGIG$ representation of $\apexgraphthree{H}$ into a $\StabGIG$ representation of $\apexgraphseven{G}$,  and (2) to convert the $\StabGIG$ representation of $\apexgraphseven{G}$ into a
% $\StabGIG$ representation of $\apexgraph{G}$, for an arbitrary $k>7$. These operations are similar, and reduce to further subdividing one edge of $\apexgraphthree{H}$, that may be appropriately chosen, by transforming it into a path of odd length $2h+1$, for an appropriate integer $h\geq 1$. 





% Consider the $\StabGIG$ representation of $\apexgraphthree{H}$. For each edge $e\in \Ecrossedge(G)$, a 7-subdivision is performed in  $\apexgraphthree{H}$. But for each edge $e\in\Eleftedge(G)\cup\Erightedge(G)$, only a 3-subdivision is performed in $\apexgraphthree{H}$. Moreover, if $k>7$ all the original edges in $G$ are insufficiently subdivided in $\apexgraphthree{H}$ with respect to $\apexgraph{G}$. Let $e\in E(G)$ be one of the edges that are insufficiently subdivided, and assume that $e\in\Eleftedge(H)$. In the case where $e\in\Erightedge(H)$, the approach is similar, whereas in the case where $e\in\Ecrossedge(G)$ perform the same approach on the 'half-edge' of $e$ that belongs to $\Eleftedge(H)$. In  $\apexgraphthree{H}$, $e$ is 3-subdivided. Assume we need a $k$-subdivision of $e$, with odd $k\geq 7$, and let $h=(k-3)/2$. Then we perform a $2h$-subdivision of the edge $(u_e^1,u_e^2)$ of $\apexgraphthree{H}$,
% and describe below the new segments representing $u_e^1, u_e^2$ and the $2h$ supplementary vertices. 

% In $\apexgraphthree{H}$, the intersection point between the segments  $\curve{u_e^3}$ and $\curve{u_e^2}$ is $(\lefty_e,\lefty_e)$. The closest possible similar point located on the stabbing line towards right is the point $(\lefty_e+\varepsilon,\lefty_e+\varepsilon)$. We then replace the segment $\curve{u_e^2}$ by a succession of $2h+1$ alternating horizontal and vertical segments whose intersections define the path required by the $2h$-subdivision of 
% $(u_e^1,u_e^2)$.

% Formally, let $\varepsilon_2=\varepsilon/(h+1)$, and define the following segments, the first of which is the new $\curve{u_e^2}$. Here, $t$ is an integer with $0\leq t\leq h-1$.
% \bigskip

% $\left((\lefty_e,\lefty_e),(\lefty_e+\varepsilon_2,\lefty_e)\right)$

% $\left((\lefty_e+\varepsilon_2,\lefty_e), (\lefty_e+\varepsilon_2,\lefty_e+\varepsilon_2)\right)$

% $\left((\lefty_e+\varepsilon_2,\lefty_e+\varepsilon_2), (\lefty_e+2\varepsilon_2,\lefty_e+\varepsilon_2)\right)$

% $\left((\lefty_e+2\varepsilon_2,\lefty_e+\varepsilon_2), (\lefty_e+2\varepsilon_2,\lefty_e+2\varepsilon_2)\right)$

% $\ldots$

% $\left((\lefty_e+t\varepsilon_2,\lefty_e+t\varepsilon_2), (\lefty_e+(t+1)\varepsilon_2,\lefty_e+t\varepsilon_2)\right)$

% $\left((\lefty_e+(t+1)\varepsilon_2,\lefty_e+t\varepsilon_2), (\lefty_e+(t+1)\varepsilon_2,\lefty_e+(t+1)\varepsilon_2)\right)$

% $\ldots$

% $\left((\lefty_e+h\varepsilon_2,\lefty_e+h\varepsilon_2), (\righty_e,\lefty_e+h\varepsilon_2)\right)$
% \bigskip

% \rt{Note: may be written without dots, but is it really comprehensible this way?}


% We may also modify $\curve{u_e^1}$ by replacing it with  $\left((\righty_e,\lefty_e+h\varepsilon_2), (\righty_e,i-1)\right)$, but this is not really necessary.

% All the segments corresponding to the $2h$ new subdivision vertices lie strictly below the closest upper segment not involved in the subdivision of $e$ (whose $y$-coordinate is at least $\lefty_e+\varepsilon$), and (not strictly) above the former segment $\curve{u_e^2}$. They also lie strictly between the $x$-coordinates of $\curve{u_e^3}$ and $\curve{u_e^1}$. So they cannot intersect other segments. So we have represented the path with $(2h+1)$ edges required by the subdivision.



% %For this, we will show that if we are given a $\StabGIG$ representation of a graph in which a particular edge (say $e$) is subdivided $r$ times (for some odd number $r$), then we can easily convert it into a $\StabGIG$ representation in which $e$ is subdivided $r+2$ times. \rt{I wonder if this is the best thing to do. If adding two segments needs to divide a small distance by $2$, then adding $2h$ segments needs to divide the same distance by $2^h$ ... and then there may be problems with the representation of very small numbers. Going from a r-subdivision to a $r+2h$ subdivision, directly, is maybe better. I have to think about it}
% \end{proof}






% % \begin{proof} $G$ is planar and subdivision does not affect planarity, so $\subdivide{G}$ is also planar, implying $\apexgraph{G}$ is an apex graph. The vertex set of $\apexgraph{G}$ can be expressed as the disjoint union of two sets $A$ and $B$, where
% % 	\begin{align*}
% % 	A &= \{x\mid x\in V(G) \}\cup\{u^i_e\mid e\in E(G), i\in[k] \text{ and $i$ is even}\};\\
% % 	B &= \{a\} \cup \{u^i_e\mid e\in E(G), i\in[k] \text{ and $i$ is odd}\}.
% % 	\end{align*}
% % 	Note that $A$ induces an independent set in $\apexgraph{G}$ (since $k$ is odd), and so does $B$. Therefore, $\apexgraph{G}$ is a bipartite apex graph. As for the girth of $\apexgraph{G}$, it is easy to see that every cycle in $\apexgraph{G}$ contains at least $k+2$ vertices $(x, u^1_e, u^2_e, u^3_e, \ldots, u^k_e, y)$, for some $e=(x,y)\in E(G)$. At least one more vertex is needed to complete the cycle, implying that the girth of $\apexgraph{G}$ is at least $k+3\geq g$.
% % \end{proof}

% \begin{proof}(of Theorem \ref{thm:stabbable-GIG})
% For a given graph $\Gamma$, recall (see Section \ref{subsec:theproofs}) that $\Gamma+x$ is the graph obtained by adding a new vertex $x$ to $\Gamma$ such that $x$ is adjacent to all the vertices in $\Gamma$. In order to show that {\sc StabGIGRec} belongs to NP, note that 
% a grid representation of $\Gamma$ in which all the segments are stabbed by the same line  $\ell$ may be seen as a representation in the plane of $\Gamma+x$ with segments following at most three directions ($x$ is represented by the stabbing 
% line $\ell$, that is replaced in this representation with a long segment).
% This remark allows us to invoke once again the result in \cite{kratochvil1994intersection}, which guarantees that since the number of directions of the segments in the representation is fixed, {\sc StabGIGRec} is in NP. \

% % rt{Would it be possible to check that my interpretation of the result in \cite{kratochvil1994intersection} is correct, and thus that the use I make here is correct too, please?} 

% % \textcolor{blue}{Using the result of \cite{kratochvil1994intersection} is correct. }

% Furthermore, $\apexgraph{G}$ is obtained in polynomial time from $G$ and Propositions \ref{prop:forward} and \ref{prop:backward} show that our reduction is correct. 
% \end{proof}











% % \rotatebox{90}{
% 			% 	\begin{tikzpicture}
				
				
% 			% 	\draw[thick] (0,0) -- (7,0);
				
% 			% 	\filldraw[blue!60!white] (4,0) circle (4pt);
% 			% 	\filldraw[blue!60!white] (3,0) circle (4pt);
% 			% 	\filldraw[blue!60!white] (2,0) circle (4pt);
% 			% 	\filldraw[blue!60!white] (1,0) circle (4pt);
% 			% 	\filldraw[blue!60!white] (0,0) circle (4pt);
% 			% 	\filldraw[blue!60!white] (5,0) circle (4pt);
% 			% 	\filldraw[blue!60!white] (6,0) circle (4pt);
% 			% 	\filldraw[blue!60!white] (7,0) circle (4pt);
				
% 			% 	\node[left] at (0.3,1.04) {\rotatebox{270} {$(v_1)$}};
				
% 			% 	\node[left] at (1.3,1.04) {\rotatebox{270} {$(v_2)$}};
				
% 			% 	\node[left] at (2.3,1.04) {\rotatebox{270} {$(v_3)$}};
				
% 			% 	\node[left] at (3.3,1.04) {\rotatebox{270} {$(v_4)$}};
				
% 			% 	\node[left] at (4.3,1.04) {\rotatebox{270} {$(v_5)$}};
				
% 			% 	\node[left] at (5.3,1.04) {\rotatebox{270} {$(v_6)$}};
				
% 			% 	\node[left] at (6.3,1.04) {\rotatebox{270} {$(v_7)$}};
				
% 			% 	\node[left] at (7.3,1.04) {\rotatebox{270} {$(v_8)$}};
				
% 			% 	\node[left] at (0.3,-1.14) {\rotatebox{270} {$(v_1)$}};
				
% 			% 	\node[left] at (1.3,-1.14) {\rotatebox{270} {$(v_2)$}};
				
% 			% 	\node[left] at (2.3,-1.14) {\rotatebox{270} {$(v_3)$}};
				
% 			% 	\node[left] at (3.3,-1.14) {\rotatebox{270} {$(v_4)$}};
				
% 			% 	\node[left] at (4.3,-1.14) {\rotatebox{270} {$(v_5)$}};
				
% 			% 	\node[left] at (5.3,-1.14) {\rotatebox{270} {$(v_6)$}};
				
% 			% 	\node[left] at (6.3,-1.14) {\rotatebox{270} {$(v_7)$}};
				
% 			% 	\node[left] at (7.3,-1.14) {\rotatebox{270} {$(v_8)$}};
				
				
				
				
% 			% 	\end{tikzpicture}} & \multicolumn{2}{c}{ \begin{tikzpicture}
% 			% 	\draw[magenta!70!black, ultra thick] (0,7) -- (0,0);
				
% 			% 	\draw[blue!60!white] (0,6.5) -- (-1.5,6.5);
% 			% 	\draw[blue!60!white] (0,5.7) -- (2.6,5.7);
% 			% 	\draw[blue!60!white] (-0.7,4.9) -- (1,4.9);
% 			% 	\draw[blue!60!white] (-2.6,4.1) -- (0.5,4.1);
% 			% 	\draw[blue!60!white] (-2,3.3) -- (0,3.3);
% 			% 	\draw[blue!60!white] (-1.4,2.5) -- (0,2.5);
% 			% 	\draw[blue!60!white] (-0.7,1.7) -- (2,1.7);
% 			% 	\draw[blue!60!white] (-1.4,0.9) -- (0,0.9);
				
% 			% 	% Cross over edges
				
% 			% 	\draw[magenta!70!black,densely dashed] (2.5,5.8) -- (2.5,-1.1);
% 			% 	\draw[magenta!70!black,densely dashed] (2.6,-1) -- (-2.6,-1);
% 			% 	\draw[magenta!70!black,densely dashed] (-2.5,-1.1) -- (-2.5,4.2);
				
% 			% 	\draw[magenta!70!black,densely dashed] (1.9,1.8) -- (1.9,-0.6);
% 			% 	\draw[magenta!70!black,densely dashed] (2,-0.5) -- (-2,-0.5);
% 			% 	\draw[magenta!70!black,densely dashed] (-1.9,-0.6) -- (-1.9,3.4);
				
% 			% 	% left edges
				
% 			% 	\draw[magenta!70!black,densely dashed] (1.7,5.8) -- (1.7,3.8);
% 			% 	\draw[magenta!70!black,densely dashed] (1.6,3.9) -- (1.6,1.6);
% 			% 	\draw[magenta!70!black,densely dashed] (1.5,3.85) -- (1.8,3.85);
				
% 			% 	\draw[magenta!70!black,densely dashed] (0.9,5) -- (0.9,3.2);
% 			% 	\draw[magenta!70!black,densely dashed] (0.8,3.3) -- (0.8,1.6);
% 			% 	\draw[magenta!70!black,densely dashed] (0.7,3.25) -- (1,3.25);
				
% 			% 	\draw[magenta!70!black,densely dashed] (0.4,4.2) -- (0.4,2.5);
% 			% 	\draw[magenta!70!black,densely dashed] (0.3,2.6) -- (0.3,1.6);
% 			% 	\draw[magenta!70!black,densely dashed] (0.2,2.55) -- (0.5,2.55);
				
				
% 			% 	% Right edges
				
% 			% 	\draw[magenta!70!black,densely dashed] (-0.4,6.6) -- (-0.4,5.8);
% 			% 	\draw[magenta!70!black,densely dashed] (-0.5,5.9) -- (-0.5,4.8);
% 			% 	\draw[magenta!70!black,densely dashed] (-0.6,5.85) -- (-0.3,5.85);
				
% 			% 	\draw[magenta!70!black,densely dashed] (-1.3,6.6) -- (-1.3,5.2);
% 			% 	\draw[magenta!70!black,densely dashed] (-1.4,5.3) -- (-1.4,4);
% 			% 	\draw[magenta!70!black,densely dashed] (-1.5,5.25) -- (-1.2,5.25);
				
% 			% 	\draw[magenta!70!black,densely dashed] (-0.4,2.6) -- (-0.4,2);
% 			% 	\draw[magenta!70!black,densely dashed] (-0.5,2.1) -- (-0.5,1.6);
% 			% 	\draw[magenta!70!black,densely dashed] (-0.6,2.05) -- (-0.3,2.05);
				
% 			% 	\draw[magenta!70!black,densely dashed] (-0.4,1.8) -- (-0.4,1.3);
% 			% 	\draw[magenta!70!black,densely dashed] (-0.5,1.4) -- (-0.5,0.8);
% 			% 	\draw[magenta!70!black,densely dashed] (-0.6,1.35) -- (-0.3,1.35);
				
% 			% 	\draw[magenta!70!black,densely dashed] (-1.2,2.6) -- (-1.2,1.6);
% 			% 	\draw[magenta!70!black,densely dashed] (-1.3,1.7) -- (-1.3,0.8);
% 			% 	\draw[magenta!70!black,densely dashed] (-1.1,1.65) -- (-1.4,1.65);
				
% 			% 	\node[above,blue!60!white] at (-1,6.5) {\large $\curve{v_8}$};
% 			% 	\node[above, blue!60!white] at (2,5.7) {\large $\curve{v_7}$};
% 			% 	\node[above,blue!60!white] at (1,4.9) {\large $\curve{v_6}$};
% 			% 	\node[above, blue!60!white] at (-2.1,4.1) {\large $\curve{v_5}$};
% 			% 	\node[above, blue!60!white] at (-1.5,3.3) {\large $\curve{v_4}$};
% 			% 	\node[above, blue!60!white] at (-1,2.5) {\large $\curve{v_3}$};
% 			% 	\node[below, blue!60!white] at (1,1.7) {\large $\curve{v_2}$};
% 			% 	\node[below, blue!60!white] at (-1,0.95) {\large $\curve{v_1}$};
				
% 			% 	\node[above,magenta!70!black] at (0,7) {\LARGE $\curve{a}$};
% 			% 	\end{tikzpicture}} \\
% 			% (d) & \multicolumn{2}{c}{(e)}
